Evaluating Creativity and Deception in Large Language Models: A Simulation Framework for Multi-Agent Balderdash

Large Language Models (LLMs) have shown impressive capabilities in complex tasks and interactive environments, yet their creativity remains underexplored. This paper introduces a simulation framework utilizing the game Balderdash to evaluate both the creativity and logical reasoning of LLMs. In Balderdash, players generate fictitious definitions for obscure terms to deceive others while identifying correct definitions. Our framework enables multiple LLM agents to participate in this game, assessing their ability to produce plausible definitions and strategize based on game rules and history. We implemented a centralized game engine featuring various LLMs as participants and a judge LLM to evaluate semantic equivalence. Through a series of experiments, we analyzed the performance of different LLMs, examining metrics such as True Definition Ratio, Deception Ratio, and Correct Guess Ratio. The results provide insights into the creative and deceptive capabilities of LLMs, highlighting their strengths and areas for improvement. Specifically, the study reveals that infrequent vocabulary in LLMs' input leads to poor reasoning on game rules and historical context (https://github.com/ParsaHejabi/Simulation-Framework-for-Multi-Agent-Balderdash).

==> tables/voting_example.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{llc}
        \toprule
         \textbf{Generator} & \textbf{Definition} & \textbf{Vote}\\ \hline
         Dictionary & Ireland ostentatiously pious person. & - \\ \hline
         Llama & \makecell[l]{An archaic term for a type of primitive drumming instrument used in \\ancient ritual ceremonies, characterized by its distinctive resonance \\and rhythmic patterns.} & Phi \\ \hline
         
         Phi & \makecell[l]{An elusive insect native to South America, the crawthumper is \\characterized by its remarkably powerful hind legs that allow it to leap \\great distances, much like a grasshopper.} & Dictionary \\ \hline
         Gemma & \makecell[l]{A sentient, subterranean creeper manipulating the tides through\\ sonic resonance, sculpting landscapes in accordance with its ethereal will.} & Phi \\ \hline
         Mistral & \makecell[l]{A traditional Scottish musical instrument, resembling a dulcimer, that \\was popular in the 18th century and believed to have soothing, therapeutic \\effects on rheumatism and arthritis.} & Llama \\ \bottomrule
    \end{tabular}
    \caption{An example of all models participating in the voting phase for ``All Balderdash'' dataset. }
    \label{tab:my_label}
\end{table*}
